MultiSegVA: Using Visual Analytics to Segment Biologging Time Series on Multiple Scales

Segmenting biologging time series of animals on multiple temporal scales is an essential step that requires complex techniques with careful parameterization and possibly cross-domain expertise. Yet, there is a lack of visual-interactive tools that strongly support such multi-scale segmentation. To close this gap, we present our MultiSegVA platform for interactively defining segmentation techniques and parameters on multiple temporal scales. MultiSegVA primarily contributes tailored, visual-interactive means and visual analytics paradigms for segmenting unlabeled time series on multiple scales. Further, to flexibly compose the multi-scale segmentation, the platform contributes a new visual query language that links a variety of segmentation techniques. To illustrate our approach, we present a domain-oriented set of segmentation techniques derived in collaboration with movement ecologists. We demonstrate the applicability and usefulness of MultiSegVA in two real-world use cases from movement ecology, related to behavior analysis after environment-aware segmentation, and after progressive clustering. Expert feedback from movement ecologists shows the effectiveness of tailored visual-interactive means and visual analytics paradigms at segmenting multi-scale data, enabling them to perform semantically meaningful analyses. A third use case demonstrates that MultiSegVA is generalizable to other domains.

==> content/02-relatedwork.tex <==

\section{Related Work}
\label{sec:relatedwork}
This section backs up the elicited requirements, contextualizes, and further motivates our work. We initially refer to techniques for time series segmentation, before depicting VA approaches for a visual-interactive segmentation process and outlining related VQLs. 
\subsection{Techniques for Time Series Segmentation}
\phil{to-do: slightly stronger focus on segmenting biologging ts + more compact}
\textbf{Single-Scale.} Many segmentation techniques are applied on a single scale with global parameters and return a single-scale alignment of segments. Keogh et al. present a segmentation survey \cite{keogh2004segmenting} with bottom-up, top-down, sliding-window algorithms, next to the efficient hybrid \textit{SWAB}, that try to meet segmentation criteria (e.g., minimum error) regarding piecewise linear approximations.

Often change point detection is applied for time series segmentation. As described in the survey of Troung et al. \cite{truong2018review} (cf. \cite{chen2013parametric, eckley2011analysis,aminikhanghahi2017survey}), the detection is usually determined by a cost function (e.g., maximum-likelihood-based, kernel-based), a search function (e.g., the optimal PELT, approximate functions as above), and additional constraints (e.g., to steer the number of change points). %In particular when segmenting geospatial time series, the related concept of stop point detection becomes important [...]. 

With stronger foundations in probability theory, Hidden Markov Models \cite{rabiner1989tutorial, zucchini2017hidden, cappe2006inference}, Hidden Semi-Markov Model, and State Space Models (SSMs) are alternatives that can capture inherent semantics better than previous techniques.

Next to the generic techniques above, there are also more domain- and data-specific techniques for, e.g., trajectory, human motion, or audio data. Furthermore, segmentation techniques with relatively different ways of functioning have recently emerged: e.g., semantic segmentation based on matrix profiles (i.e., nearest-neighbor curves, cf. \cite{gharghabi2017matrix}), motion segmentation based on graphs REF. Finally, a common aspect of above techniques is that their standard variants do not strongly address the multi-scale character of time series, as they are often applied on a single time scale with global parameters.

\phil{cf. Analysis and visualisation of movement: an interdisciplinary review}
\textbf{Multi-Scale.} The multi-scale character of time series becomes emphasized by more complex variants of previous techniques, e.g., by  hierarchical HMM, multilevel SSM, multi-scale change point detection \cite{dette2018multiscale, frick2014multiscale}. For example, Cho and Fryzlewicz propose a non-parametric Wavelet model \cite{cho2012multiscale} to identify change points in periodograms of multiple scales. In general, alternative approaches can emerge from the field of multi-scale time series modeling \cite{ferreira2006multi, ferreira2007multiscale}. Thus to identify the multi-scale structure of a time series, Vamoş proposes a technique \cite{vamocs2017multiscale} based on a time series' monotony spectrum: i.e., "the variation of the mean amplitude of the monotonic segments
with respect to the mean local time scale during successive averagings of the time series"\cite{vamocs2017multiscale}. Such techniques have strong theoretical foundations and their overall value is certainly inquestionable. Though, their increased complexity demands (a) stronger efforts at parametrization 
and (b) thorough (cross-)domain expertise in statistics. Having these hindering factors, the next subsection regards to which extent visual-interactive approach could support the analyst at multi-scale segmentation. 
%\begin{itemize}
 %\item \phil{contextualize+ motivate; not into algorithmic details; difficulties of multi-scale techniques?}
  %  \item (wavelet decomposition; and multi-scale models prominent at time series forecasting) 
   % \item hierarchical segmentation of human motion data based on k-means, \cite{zhou2013hierarchical}
    %\item Temporal Scale Selection in Time-Causal Scale Space
    %\item transition to vis
%\end{itemize}
\subsection{VA approaches for Time Series Segmentation}
\label{sec:relva}
\begin{table}[h!t]
  \centering
  \includegraphics[width=.95\linewidth]{images/relatedtable.png}
  \caption{Comparison of related approaches. Note that no related approach fulfills \textbf{R3} and \textbf{R4} specifically in the multi-scale setting.  }
  \label{tbl:vacomparison}
  \vspace{-1\baselineskip}
\end{table}

The following VA approaches shall enable interactive time series segmentation, where "humans and machines
cooperate using their respective distinct capabilities for the most effective results" \cite{keim2008visual}. Note that several of these approaches are originally intended for movement and motion analyses. 

Spretke et al. present their VA tool \textit{AnimalEcologyExplorer} \cite{spretke2011exploration}, while emphasizing that VA "can help to empower the animal tracking community and to foster new insight into the ecology and movement of tracked animals" \cite{spretke2011exploration}. AnimalEcologyExplorer is intended for the iterative enrichment and segmentation of animal movement time series. The outcomes are visually encoded in trajectory views, horizon graphs and line charts, and can be refined within a strong feedback loop. However, AnimalEcologyExplorer enables only simple value range segmentation that is applied on a single scale.  

Alsallakh et al. describe a VA approach \cite{alsallakh2014visual} where the user decides between different segmentation techniques and parameters. The user specifies intervals for the local application of the chosen techniques, observes outcomes in interactive visualizations, and can follow a feedback loop. In principle, the local application allows segmentation on multiple and nested temporal scales, but the proposed one-dimensional color stripe visualization does not strongly support multi-scale analyses. \phil{Make more compact:}\daniel{The \textit{KronoMiner} system proposed by Zhao et al.~\cite{zhao2011kronominer} offers more flexible and generalizable time series analysis and segmentation capabilities on multiple scales. Using a hierarchical circular layout, users can compare multiple multivariate time series datasets and can interactively segment them on several levels. The individual segments can be investigated and compared in detail using either detail views or the so-called \textit{Magic-Analytics} lens. \textit{KronoMiner} is an approach that allows for segmenting time-series on multiple scales; however, this is a fully manual approach that only allows for segmenting and generating a hierarchy tree based on user-defined time ranges. Thus finding insights, especially on lower levels, is a complex task, since identifying the corresponding segments in multiple time series and comparing them is an entirely exploratory approach.}

Röhlig et al. \cite{rohlig2015parameters} enable the analysis of the impact of different parameter configurations in an interactive prototype.  Here, a time series is segmented multiple times with differently parametrized SSMs. The segmentation results are encoded by juxtaposed color stripes, having several possible color encodings, aggregation and interaction techniques. Though, neither a multilevel SSM nor local or multi-scale parameter impacts are considered by the described approach. 

Further approaches do not consider typical segmentation techniques inherently, but still help structuring the time series by the help of VA principles. The \textit{TimeClassifier} tool \cite{walker2015timeclassifier} of Walker et al. structures time series via template matching and visually encodes confidence scores of matched segments. A web tool \cite{gao2013web} of Gao et al. identifies and annotates segments by a hierarchical support vector machine (SVM). This web tool is intended for biologging time series, shall distinguish high and low level motion patterns, but has few visual-interactive features. %\textit{MotionExplorer} \cite{MotionExplorer} of Bernard et al. allows interactive hierarchical clustering of human poses, then to identify motion sequences after having specified start and end poses in a search interface. 

The above related VA approaches can be compared to MultiSegVA directly, shown in Figure~\ref{tbl:vacomparison}. Besides the requirements as defined in Section~\ref{sec:tasks}, we also take into consideration, whether an approach supports multivariate data, whether it is generalizable to arbitrary time series data and whether it supports a geospatial context of the displayed data. From the table, it is apparent that the support for different hierarchies in combination with flexible segmentation and spatial context analysis is limited, especially for multivariate data.
Further distinction would be possible by comparing the scalability of techniques with respect to temporal resolution of data points, duration and amount of different time series to be analyzed in context. Yet, these properties are not described completely in all compared works. The range for amount of displayable time series goes from 1 with high temporal resolution and a duration of a few hours of data for Walker et al.~\cite{walker2015timeclassifier} to many, but with restricted temporal resolution as for Spretke et al.~\cite{spretke2011exploration}. To the best of our knowledge, we have found no tool that scales to multiple time series with high temporal resolutions (>1 Hz) over longer durations than a few hours. Finally, spatial references play a vital role in many use cases, such as described in Section~\ref{sec:eval}. The comparison shows, that only few related approaches are able to relate time series to spatial positions.

Consequently, to the best of the authors' knowledge, there is no VA approach that simultaneously puts strong emphasis on \textit{true \juri{Das m\"usste man doch nochmal definieren ;)}} time series segmentation and the analysis on multiple temporal scales. To fill this gap, this publication describes a VA system that includes an new visual query language for multi-scale time series segmentation. 

\subsection{Visual Query Languages}

Visual query languages (\textit{VQL}) allow a wide range of users to search records or databases by replacing queries and the structure of the data with visual representations, thus offloading the complexity of query creation from the user to the system. An example for a VQL is the VISAGE Querying Language \cite{pienta2016visage} that enables the visual-interactive querying of graph databases. 

Despite  many efforts in the research area of VQL approaches and many existing application examples, there is still a need for further research, especially in the area of query languages for temporal domains~\cite{Catarci2009}. The main focus of current research in the field of visual query languages for the temporal domain lies currently on event sequences. Examples for this are numerous. Decisionflow\cite{gotz2014decisionflow} is a visual analytics solution for high-dimensional temporal event sequence data , that provides a visual query interface to find event sequences by specifying preconditions, episodes and outcomes. not hierarchical, only works for event based temporal data or a related approach by Kraus et al.~\cite{krause2015supporting} that allows for the visual-interactive segmentation and filtering of event sequences.% (\daniel{The \textit{TimeSlice} presented by Zhao et al.~\cite{zhao2012timeslice} allows for the faceted browsing of timeline data by hierarchically creating user-defined faceted views on the data. However, these faceted views can only be based on predefined categorical attributes of the timeline data, such as gender or profession.}) 
One approach that focuses on segmenting is Segmentifier~\cite{dextras2019segmentifier}, which iteratively applys filter operations to refine and subdivide click-stream sequence data into smaller segments via attribute and pattern constraints for further detailed inspection. However, all of these aforementioned approaches focus on event sequences and not unlabeled time series data. One approach that works with unlabeled movement trajectories, a form of multivariate time series data, is the one presented by Stein et al.~\cite{stein2019movement}, which enables the hierarchical composition of events from the raw movement data using a visual query interface. However, the proposed approach only focuses on movement data and doesn't consider hierarchical segmentation. 


%\subsection{Positioning}
%\label{sec:vql}
%
%\begin{itemize}
%    \item EuroVA short paper: choice of different methods/parameters (Bernard, \cite{bernard2016visual}
%    \item EuroVA short paper: conceptualization segmentation workflow (Bernard, \cite{bernard2018pipeline})
%\end{itemize}

